The Limits of an Information Intermediary in Auction Design

We study the limits of an information intermediary in the classical Bayesian auction, where a revenue-maximizing seller sells one item to $n$ buyers with independent private values. In addition, we have an intermediary who knows the buyers' private values, and can map these to a public signal so as to increase consumer surplus. This model generalizes the single-buyer setting proposed by Bergemann, Brooks, and Morris, who present a signaling scheme that raises the optimal consumer surplus, by guaranteeing that the item is always sold and the seller gets the same revenue as without signaling. Our work aims to understand how this result ports to the setting with multiple buyers. We likewise define the benchmark for the optimal consumer surplus: one where the auction is efficient (i.e., the item is always sold to the highest-valued buyer) and the revenue of the seller is unchanged. We show that no signaling scheme can guarantee this benchmark even for $n=2$ buyers with $2$-point valuation distributions. Indeed, no signaling scheme can be efficient while preserving any non-trivial fraction of the original consumer surplus, and no signaling scheme can guarantee consumer surplus better than a factor of $\frac{1}{2}$ compared to the benchmark. These impossibility results are existential (beyond computational), and provide a sharp separation between the single and multi-buyer settings. In light of this impossibility, we develop signaling schemes with good approximation guarantees to the benchmark. Our main technical result is an $O(1)$-approximation for i.i.d. regular buyers, via signaling schemes that are conceptually simple and computable in polynomial time. We also present an extension to the case of general independent distributions.

==> upper.tex <==
% !TEX root = ms.tex
\section{An $O(\log n)$ Approximation of Consumer Surplus}


For any distribution $D$, we write $F_D(v) = \Pr_{V \sim D}[V \geq v]$ and $f_D(v) = \Pr_{V \sim D}[V = v]$. Let $r_i$ be the smallest optimal reserve price that maximizes $r \cdot F_{X_i}(r)$. Define $p_i := 1 - F_X(r)$.

\begin{theorem}
The signaling scheme above is an $O(\log n)$ approximation for the consumer surplus.
\end{theorem}
\begin{proof}
We will construct a set of signaling schemes each associated with a weight, and show the total weighted CS is at least $\opt$ and the total weight is $O(\log n)$. By using each signaling scheme with probability proportional to its weight, we will get an $O(\log n)$ approximation.

The first signaling scheme with weight $1$ is to send no additional information. The seller will just run Myerson's auction and we will get Myerson's CS from this scheme. This scheme may not be efficient because
\begin{enumerate}
\item sometimes the item may not be allocated to anyone, and
\item sometimes the item is allocated, but not to the buyer with the highest valuation.
\end{enumerate}
The first case only happens if all items are below their respective reserve prices, and the CS lost here is
\[
T_1 := \left(\prod_{i = 1}^n p_i \right) \cdot \E_{V_i \sim X_i}\left[\max_{i = 1, 2, \ldots, n} V_i \ \middle|  \ \forall i, \ V_i < r_i\right].
\]
The second case happens if someone has positive virtual value, but the buyer with the highest virtual value is not the buyer with the highest value. The CS lost in this case is
\[
T_2 := \sum_{i = 1}^n \Pr[i\text{ has the largest virtual value and }> 0] \cdot \E[\max_{j = 1, 2, \ldots, n} V_j - V_i \mid i\text{ has the largest virtual value and }> 0].
\]

We deal with $T_1$ and $T_2$ separately in the following discussion.

\paragraph{Approximation of $T_1$.} Define $Y_i$ to be the conditional distribution of $X_i$ strictly below $r_i$. (If some $p_i = 0$, $T_1 = 0$. Thus we assume $p_i > 0$ and $Y_i$'s are well defined.) We make $n$ independent draws, where the $i$-th draw is from $Y_i$, and let $Z_t$ denote the distribution for the $t$-th largest value among them. We now rewrite $T_1$ as
\[
T_1 = \left(\prod_{i = 1}^n p_i \right) \cdot \E[Z_1].
\]

Now we consider the following signaling scheme: We reveal the realized valuations for all but the $k$ largest. Define the $(k+1)$-th highest valuation to be $\bar v \in \mathbb{R}$. ($\bar v = 0$ if $k = n$.) For the buyers with the top $k$ valuations, we randomly pick one, and do BBM on its valuation minus $\bar v$.

The seller, upon receiving the signal, observes the following information:
\begin{itemize}
\item The realized valuations of $n - k$ buyers, the highest of which is $\bar v$.
\item The valuation distributions of $k - 1$ buyers. Each of them is $X$ conditioned on being greater than $\bar v$, and they are independent.
\item The valuation distribution of the randomly picked buyer. It is also independent from the $k - 1$ distributions above. After subtracting $\bar v$ from it, it is an equal-revenue distribution.
\end{itemize}
The optimal strategy for the seller is to subtract $\bar v$ from all valuations, run Myerson's auction on the top $k$ buyers, and sell to the buyer with valuation $\bar v$ (before the subtraction) if the item is not sold. Myerson's auction on the top $k$ buyers will be sold to the randomly selected buyer if the $k - 1$ distributions are below the new optimal reserve price $r'$.

\begin{lemma}
The optimal reserve price of the distribution $D_{| > \bar v} - \bar v$ is at least $r - \bar v$, where $r$ is the smallest optimal reserve price of $D$.
\end{lemma}
\begin{proof}
Let $D' = D_{| > \bar v} - \bar v$. Suppose for contradiction that for some $r' < r - \bar v$,
\[
r' \cdot F_{D'}(r') \geq (r - \bar v) \cdot F_{D'}(r - \bar v).
\]
Then we will have
\[
(r' + \bar v) \cdot F_{D'}(r') \geq r \cdot F_{D'}(r - \bar v),
\]
since $F_{D'}(r') \geq F_{D'}(r - \bar v)$. Thus,
\[
(r' + \bar v) \cdot F_{D}(r + \bar v) \geq r \cdot F_{D'}(r),
\]
a contradiction to the assumption that $r$ is the smallest optimal reserve price of $D$.
\end{proof}
Let $b$ be the randomly selected buyer for BBM. Let $A(\mathbf{v}, b, k)$ be the event that $v_b > \kth{\mathbf{v}}{k + 1}$. The CS of our signaling scheme is at least
\begin{align*}
&\sum_{b = 1}^n \sum_{\mathbf{v}_{-b} : v_i < r_i} \left(\prod_{i \in N \setminus \{b\}} f_{X_i}(v_i)\right) \cdot F_{X_b}\left(\kth{\mathbf{v}}{k + 1}\right) \cdot \sum_{v_b < r_b} \mathbbm{1}_{A(\mathbf{v}, b, k)} \cdot \frac{1}{k} \cdot \frac{f_{X_b}(v_b) \cdot \left(v_b - \kth{\mathbf{v}}{k + 1}\right)}{F_{X_b}\left(\kth{\mathbf{v}}{k + 1}\right)}\\
= &\sum_{b = 1}^n \sum_{\mathbf{v} : v_i < r_i} \left(\prod_{i \in N} f_{X_i}(v_i)\right) \cdot \mathbbm{1}_{A(\mathbf{v}, b, k)} \cdot \frac{1}{k} \cdot \left(v_b - \kth{\mathbf{v}}{k + 1}\right)\\
= &\left(\prod_{i \in N} p_i\right) \cdot \sum_{b = 1}^n \sum_{\mathbf{v} : v_i < r_i} \left(\prod_{i \in N} f_{Y_i}(v_i)\right) \cdot \mathbbm{1}_{A(\mathbf{v}, b, k)} \cdot \frac{1}{k} \cdot \left(v_b - \kth{\mathbf{v}}{k + 1}\right).
\end{align*}
The analysis also holds for $k = n$ if we assume $\kth{\mathbf{v}}{k + 1} = 0$ in this case.

Recall that $Z_t$ is the distribution for the $t$-th largest value among independent draws from $X_1, X_2, \ldots, X_n$. The formula above simplifies to
\begin{align*}
&\left(\prod_{i \in N} p_i\right) \cdot \sum_{\mathbf{v} : v_i < r_i} \left(\prod_{i \in N} f_{Y_i}(v_i)\right) \cdot \left((\text{average of top }k\text{ in }\mathbf{v}) - \kth{\mathbf{v}}{k + 1}\right)\\
= &\left(\prod_{i \in N} p_i\right) \cdot \left(\left(\frac{1}{k} \cdot \sum_{j = 1}^k \E[Z_j]\right) - \E[Z_{j+1}]\right).
\end{align*}

By choosing each $k = t < n - 1$ with weight $\frac{1}{t + 1}$ and $k = n - 1$ with weight $1$, we get
\begin{align*}
&\left(\prod_{i \in N} p_i\right) \cdot \left(\left(\sum_{i = 1}^{n - 2} \E[Z_i] \cdot \sum_{j = i}^{n - 2} \frac{1}{j(j+1)}\right) - \left(\sum_{i = 2}^{n - 1} \E[Z_i] \cdot \frac{1}{i}\right) + \left(\sum_{i = 1}^{n - 1} \E[Z_i] \cdot \frac{1}{n - 1}\right) - \E[Z_n]\right)\\
= &\left(\prod_{i \in N} p_i\right) \cdot (\E[Z_1] - \E[Z_n]).
\end{align*}

Notice that when $k = n$, we get at least $\left(\prod_{i \in N} p_i\right) \cdot \frac{\sum_{i = 1}^n \E[Z_i]}{n} \geq \left(\prod_{i \in N} p_i\right) \cdot \E[Z_n]$ as CS. Thus adding another signaling scheme with weight $1$ for $k = n$ will make the total weighted CS at least $\left(\prod_{i \in N} p_i\right) \cdot \E[Z_1] = T_1$. The total weight used to approximate $T_1$ is $2 + \sum_{i = 2}^{n - 1} \frac{1}{i} \leq 2 + \ln n$.

\paragraph{Approximation of $T_2$.} Consider the following signaling scheme: Let $b$ be the buyer with the highest virtual value. We reveal to the seller the identity of $b$ and her realized valuation $v_b$. %Now the seller knows each other buyer $i$ has virtual value at most $\varphi_b(v_b)$, giving a conditional distribution $X_i'(b, v_b)$, and they are still independent. The seller will use the auction as if each other buyer has valuation drawn from $X_i'(b, v_b)$ minus $v_b$, with an added price of $v_b$; and sell the item to buyer $b$ at price $v_b$ if not sold.
Among the rest $n - 1$ buyers, similar to the other case, we reveal the realized valuations but the $k$ largest ones. Let the $(k + 1)$-th largest be $\bar v \in \mathbb{R}$. We pick a random buyer among the top $k$ to do BBM on her valuation minus $\max(v_b, \bar v)$. We choose each $k = t < n - 2$ with weight $\frac{1}{t + 1}$, $k = n - 2$ with weight $1$, and $k = n - 1$ with weight $1$. Let $B(\mathbf{v}, b)$ be the event that $b = \argmax_i \varphi_i(v_i)$ and $\varphi_b(v_b) \geq 0$. By the same argument as the previous case, we gain the maximum value minus $v_b$ whenever everyone other than $b$ is below the new reserve.  Note that $\varphi_i(v_i) < \varphi_b(v_b)$ implies $\varphi_i(v_i) < v_b$ and after subtracting $v_b$ from it, the virtual value of $i$ becomes negative. Therefore we get at least
\begin{align*}
&\sum_{\mathbf{v}} \sum_{b = 1}^n \left(\prod_{i \in N} f_{X_i}(v_i)\right) \cdot \mathbbm{1}_{B(\mathbf{v}, b)} \cdot \left(\max_{i \in N} v_i - v_b\right).
\end{align*}
%Here $Y_i'(b, v_b)$ is the conditional distribution of $(X_i'(b, v_b) - v_b)$ below its new reserve. $p_i'$ is the probability that $(X_i'(b, v_b) - v_b)$ is below its new reserve.
The total weight used to approximate $T_2$ is $2 + \sum_{i = 2}^{n - 2} \frac{1}{i} \leq 2 + \ln n$.

 Using each signaling scheme with probability of its weight divided by $5 + 2\ln n$ gives an $O(\log n)$ approximation.
\end{proof}


